Heat Conduction with Phase Change in Permafrost Modules of Vegetation Models

We consider the problem of heat conduction with phase change, that is essential for permafrost modeling in Land Surface Models and Dynamic Global Vegetation Models. These models require minimal computational effort and an extremely robust solver for large-scale, long-term simulations. The weak enthalpy formulation of the Stefan problem is used as the mathematical model and a finite element method is employed for the discretization. Leveraging the piecewise affine structure of the nonlinear time-stepping equation system, we demonstrate that this system has a unique solution and provide a solver that is guaranteed to find this solution in a finite number of steps from any initial guess. Comparisons with the Neumann analytical solution and tests in the Lund-Potsdam-Jena managed Land vegetation model reveal that the new method does not introduce significantly higher computational costs than the widely used DECP method while providing greater accuracy. In particular, it avoids a known nonphysical artifact in the solution.

==> nomenclature.tex <==
\nomenclature[C]{$u(x,t)$}{The soil temperature \nomunit{°C} }
\nomenclature[C]{$e(x,t)$}{The volumetric enthalpy \nomunit{\frac{J}{m^3} }}
\nomenclature[C]{$L(x)$}{The volumetric latent heat of soil due to its water content \nomunit{ \frac{J}{m^3} } }
\nomenclature[C]{$c_u(x)$}{The volumetric heat capacity of soil in unfrozen state at depth $x$ \nomunit{ \frac{J}{m^3 K} } }
\nomenclature[C]{$c_f(x)$}{The volumetric heat capacity of soil in frozen state at depth $x$ \nomunit{ \frac{J}{m^3 K} } }
\nomenclature[C]{$q(x,t)$}{The heat flux at $x$ \nomunit{ \frac{W}{m^2} } }
\nomenclature[C]{$k_u(x)$}{The thermal conductivity of soil in unfrozen state at depth $x$ \nomunit{ \frac{W}{m K} } }
\nomenclature[C]{$k_f(x)$}{The thermal conductivity of soil in frozen state at depth $x$ \nomunit{ \frac{W}{m K} } }
\nomenclature[C]{$s(t)$}{The ground surface temperature at time $t$ \nomunit{ °C } }

